Tensor network representations of discrete maximum entropy distributions via mean polytopes

We present tensor network representations for discrete maximum entropy distributions under expectation constraints. To this end, we introduce Computation-Activation Networks (CompActNets), a tensor network architecture that subsumes exponential families. By leveraging the geometry of the convex polytope of realizable expectation vectors, we represent any maximum entropy distribution in the same architecture. We exploit the fact that proper faces of this polytope correspond to the boundary closure of exponential families, which restricts the distribution's support. We then derive explicit representations for the support within the CompActNet architecture. The proposed framework suggests tensor network ranks as complexity measures for faces. Finally, a case study on Boolean statistics links the geometry of 0/1-polytopes directly to propositional formulas.

==> info/acknowledgements.tex <==
AG and ME acknowledge funding from the German Federal Ministry of Education and Research (BMBF), grant number FKZ 13N17160, "Verbundprojekt: Quantum Read-Once-Memory - Verwandlung von klassischen Daten zu Quantenzuständen - Teilvorhaben: Quanten{\allowbreak}schaltkreis-Optimierung von Quantenzuständen durch Tensor-Netzwerke (QOQ-tn)".
ME acknowledge funding from the Deutsche Forschungsgemeinschaft (DFG, German Research Foundation) under Germany´s Excellence Strategy – The Berlin Mathematics Research Center MATH+ (EXC-2046/2, project ID: 390685689, Project PaA-7)

==> info/keywords.tex <==
Tensor networks,
Information geometry,
Maximum entropy distributions,
Mean polytopes,
Exponential families,
Neuro-symbolic AI

==> info/msc-classification.tex <==
62B10, % Statistical Information theory
68T27,   %	Logic in artificial intelligence
68T30,   %	Knowledge representation
68T37,   %	Reasoning under uncertainty in the context of artificial intelligence
15A69,   %	Multilinear algebra, tensor calculus
52B11   %	$n$-dimensional polytopes
%65F99,  %	None of the above, but in this section: Numerical linear algebra
%94A17 %	Measures of information, entropy

==> macros/implementation_macros.tex <==
%! Author = alexgoessmann
%! Date = 26.05.25

% Tandem in representation.suffixes, where the macros are strings

% Cores
\newcommand{\comCoreSuf}{\stringof{\_cC}}
\newcommand{\actCoreSuf}{\stringof{\_aC}}

\newcommand{\atoCoreSuf}{\stringof{\_atoC}}
\newcommand{\vselCoreSuf}{\stringof{\_vselC}}

% Colors
\newcommand{\disVarSuf}{\stringof{\_dV}}
\newcommand{\comVarSuf}{\stringof{\_cV}}
\newcommand{\selVarSuf}{\stringof{\_sV}}
\newcommand{\terVarSuf}{\stringof{\_tV}}

% Refiners
\newcommand{\selCoreIn}{\stringof{\_s}}

\newcommand{\eviCoreIn}{\stringof{\_e}}

\newcommand{\heaIn}{\stringof{\_h}}
\newcommand{\funIn}{\stringof{\_f}}
\newcommand{\posIn}{\stringof{\_p}}

\newcommand{\datIn}{\stringof{\_d}}



%
\newcommand{\defaultCoreType}{\inlinecode{NumpyCore}} % as in engine.core_creation
\newcommand{\defaultContractionMethod}{\inlinecode{NumpyEinsum}} % as in engine.contraction_handling

==> tikz/mean-polytope/meanset_sketch_generic.tex <==
\begin{tikzpicture}[scale=0.315]

    %% States
    \begin{scope}
        [shift={(2,18)}]

        \node[right] at (8.5,0) {$\stateset=\facstates$};

        \draw[thick] (0,0) ellipse (8cm and 2cm);
        \filldraw (-6,1.0) circle (\dotsize);
        \filldraw (-4.5,-1.3) circle (\dotsize);

        \filldraw (-1,1.8) circle (\dotsize);
        \filldraw (1,-1.8) circle (\dotsize);
        \filldraw (3.5,-1.0) circle (\dotsize);
        \filldraw (6.5,0.7) circle (\dotsize);
        \filldraw (4.5,1.4) circle (\dotsize);

        % Base measure support
        \filldraw (-3,0.6) circle (\dotsize);
        \filldraw (-1.5,0.8) circle (\dotsize);
        \filldraw (-1,-0.4) circle (\dotsize);

    \end{scope}

    \draw[->] (11,17) to[bend left=20] (11,12);% node[midway,right] {$\statepolytopemap$};
    \node[anchor=center] at (13,14.5) {$\sstatencoding$};
    \node[anchor=center] at (11.5,11) {$\genmeanset\subset\parspace$};


    \node[below] at (-1,7) {$\sbinteriorof{\genmeanset}$};

    \coordinate (A) at (0,0);

    \node[below] at (A) {$\meanparamof{1}$};
    \draw[fill] (A) circle (\dotsize);

    \coordinate (B) at (12,2.5);

    \coordinate (P2) at (2,10);
    \node[below] at (P2) {$\meanparamof{3}$};
    \draw[fill] (P2) circle (\dotsize);

    \coordinate (C) at (7.5,12);
    \path (B) -- (C) coordinate[pos=0.5] (P4);
    \path (B) -- (C) coordinate[pos=0.7] (P1);
    \node[left] at (P1) {$\meanparamof{2}$};
    \draw[fill] (P1) circle (\dotsize);


    \node[right] at (P4) {$\facesymbol$};
    \coordinate (D) at (-3,12);
    \coordinate (E) at (-10,5);

%    \node[below] at ($0.5*(A)+0.5*(E)-(0,1.3)$) {$\genmeanset/\sbinteriorof{\genmeanset}$};

    \draw[thick] (A) -- (B) -- (C) -- (D) -- (E) -- cycle;

\end{tikzpicture}


